The High-Energy Interpretation of Quantum Mechanics

We address the issue of the interpretation of quantum mechanics by asking why the issue never arises in the description of high-energy interactions. We argue that several tenets of quantum mechanics, specifically the collapse of the wave function, follow directly once one accepts the essential randomness of fundamental interaction events. We then show that scale separation of fundamental interactions ensures that decoherent measurement can be unambiguously separated from the random quantum events. Finally, we argue that the fundamental symmetries of space and time guarantee the existence of a unique preferred basis. We argue that this set of ideas might lead to an interpretation of quantum mechanics, or rather, show in which sense an "interpretation" is (or is not) necessary.

==> EJLateX/NEWS <==
REVISION HISTORY

14/06/2012 release 0.4 - first public release
27/06/2012 release 0.5 - removed the mdframed dependency in ejtex.cls (now floating envs and footnote can be used in 
			 EJarticle env). All code related to the background management is in ejbackground.sty file.
			 Minor beautify of code in ejtex.cls.
04/07/2012 release 0.6 - unreleased (initial implementation of pages 2, 3 and TOC). Introduction of fullwidth.sty 
			 and coverage.tex
05/07/2012 release 0.7 - bug's correction in ejtex.cls: global definition of \savebox, avoid reference in marks (both), 
			 no more xlxtra package use (problems with footnote numbering font size)
11/07/2012 release 1.0 - First complete release, with coverage, TOC, etc. All logo image are ok.
16/07/2011 release 1.01 - update ejtex.cls to solve a problem connected with an article that finish <exactly> at the end of a page 
			 (calculation error in tikz reference point \EJendPos). added in preamble the package "url" for better url 
			 typesetting
17/07/2011 release 1.02 - update ejtex.cls to correct the TOC line below the article title: now it's the address and not the email,
			  as in the previous issues. Defined the \EJcoverdesc (to be used in Cover.tex) to make possible the change 
			  of cover image description outside the LaTeX template. Some little correction in the second cover (Technical
			  Editor, Juan email address, LaTeX typeset). New TOC (address instead of email address) and consequent change
			  in \EJchapter signature

==> EJLateX/coverpage.tex <==
%%
%% LaTeX file for the typesetting of the cover page (1 and 2) of Euresis Journal
%%
%% www.euresisjournal.com
%%
%% Copyright (c) 2012 Davide PJ Caironi - davide dot caironi at gmail dot com
%%
%% v1.03 18/07/2012 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% cover %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\definecolor{fixedleft}{RGB}{191,204,225} %arriva fino a 121,145,155
\definecolor{blendleft}{RGB}{0,0,0}
%\definecolor{fixedright}{RGB}{205,215,231}
%\definecolor{maincolor}{RGB}{179,38,41} %arriva fino a 89,43,38 o 74,41,36 in diagonale
%\definecolor{blendmain}{RGB}{105,0,5}
\definecolor{blendmain}{RGB}{ 0,0,0}
\definecolor{cborder}{gray}{0.55}

%\tikz\shade[shading=axis,bottom color=black!10,top color=black,shading angle=-45]  (0,0) rectangle (3,3);


\thispagestyle{empty}
%\pgfdeclareimage[interpolate=false,height=135mm]{topImage}{coverImages/top.jpg}
\begin{tikzpicture}[remember picture,overlay]

	%upper left rectangle
	\node at (current page.north west) [xshift=17mm](a){};
	\node at (a) [yshift=-110mm,xshift=12mm](b){};
	%\draw[fill=fixedleft,draw=none] (a) rectangle (b);
	\shade[shading=axis,top color=fixedleft!60!blendleft,bottom color=fixedleft,draw=none] (a) rectangle (b);

	%grey bar at upper left
	\node at (b) [yshift=-44mm,xshift=1.5mm](c){};
	%\draw[fill=cborder,draw=none] (b |- a) rectangle (c);
	\shade[top color=black,bottom color=cborder,draw=none]  (b |- a) rectangle (c);

	%big gray rectangle
	\node at (a) [xshift=78mm](d){};
	\draw[fill=black!10!,draw=none] (c) rectangle (d);

	%small black rectangle
	\node at (d) [yshift=-107mm,xshift=9mm](e){};
	\draw[fill=black,draw=none] (d) rectangle (e);

	%upper main color box
	\node at (e) [yshift=52mm](f){};
	\node at (d) [xshift=26mm](g){};
	\draw[fill=maincolor,draw=none] (f) rectangle (g);

	\node at (f) [xshift=106mm,yshift=-135mm](h){};
	%\draw[fill=yellow,draw=none] (f) rectangle (h);

	%\node at (f) [yshift=-135mm,anchor= south west,draw=none,inner sep = 0pt](i){\pgfuseimage{topImage}};
	
	%\node at (f) [yshift=-135mm,anchor= south west,draw=none,inner sep = 0pt](i){\includegraphics[height=135mm,clip=true,trim=1.8cm 0 0 0]{coverImages/top.jpg}};
%	\node at (current page.south west) [] (c){};
%	\node at (c)[xshift=5.8cm,yshift=\paperheight )](d){};
%	\draw[fill=gborderB,line width=0pt,draw=gborderB] (c) rectangle (d);

	%inserire un clipping per la parte dx dell'immagine che va fuori dalla pagina... (non si sa mai)
	\node at (f) [yshift=-135mm,anchor= south west,draw=none,inner sep = 0pt](i){\EJthistopimage};

	%euresis logo
	\node at (g) [yshift=-13mm,xshift=10mm,anchor= north west,draw=none,inner sep = 0pt](j){\includegraphics[width=63mm]{EJLateX/img/Euresis_Logo_big.pdf}};

	%some position as i, but I can't use i because contains the image and anchor=south west doesn't work...
	%small rectanble at the left base of the top image
	\node at  (f) [yshift=-135mm](k){};
	\node at (k) [xshift=23mm,yshift=36mm](l){};
	\draw[fill=fixedright,draw=none] (k) rectangle (l);

	%euresis journal logo
	\node at (c) [yshift=-2mm,xshift=-14mm,anchor= north west,draw=none,inner sep = 0pt](m){\includegraphics[width=84mm]{EJLateX/img/EJournal.png}};

	%main color rectangle on top of top image, containing volume and date issue
	\node at (k) [yshift=36mm](n){};
	\node at (n) [yshift=42mm,xshift=46mm](o){};
	%\draw[fill=maincolor,draw=none] (n) rectangle (o);
	\shade[shading=axis,bottom color=maincolor!40!blendmain,top color=maincolor,shading angle=-45,draw=none] (n) rectangle (o);

%\tikz\shade[shading=axis,bottom color=black!10,top color=black,shading angle=-45]  (0,0) rectangle (3,3);


	\node at (n)[anchor= south west,draw=none,inner sep = 8pt] (p) {
		\begin{minipage}[r]{4cm}
			{\color{white} \LARGE{\textit{\hspace{-1mm}Volume \EJthisissue}}\\
			\normalsize{\textit{\EJthisdate}}}
		\end{minipage}
	};

	%\node at (current page.south west) [anchor= south west,draw=none,inner sep = 0pt](q){\adjincludegraphics[trim=5mm 6cm 0mm 14.1cm,clip,height=107mm]{coverImages/bottom.jpg}};
	
	%bottom image
	\node at (k |- current page.south west) [anchor= south east,draw=none,inner sep = 0pt](q){\EJthisbottomimage};
	
	%bottom image blank mask at bottom
	\node at (current page.south west)[xshift=105mm](r){};
	\node at (current page.south west)[xshift=31.3mm,yshift=14mm](s){};
	\draw[fill=white,draw=none] (r) rectangle (s);

	%bottom image blank mask at top left
	\node at (current page.south west)[yshift=117mm](x){};
	\node at (current page.south west)[xshift=30mm,yshift=59mm](y){};
	\draw[fill=white,draw=none] (x) rectangle (y);

	%main color rectangle on lower top of bottom image
	\node at (current page.south west)[xshift=18mm](t){};
	\node at(t)[yshift=77mm,xshift=12mm](u){};
	%\draw[fill=maincolor,draw=none] (t) rectangle (u){};
	\shade[shading=axis,bottom color=maincolor!40!blendmain,top color=maincolor,draw=none] (t) rectangle (u){};;

	%grey bar at down left
	\node at(s)[yshift=-14mm](v){};
	\node at(u)[yshift=30.1mm](w){};
	\%draw[fill=cborder,draw=none] (v) rectangle (w){};
	\shade[bottom color=black,top color=cborder,draw=none]  (v) rectangle (w){};

	%small bar at the right of the logo, down right
	\node at (current page.south east)[xshift=-11mm](z){};
	\node at (current page.south east)[xshift=-11.1mm,yshift=68mm](A){};
	\draw[fill=cborder,draw=none] (z) rectangle (A);

	%logo(s)
	\node at (current page.south east)[xshift=-50mm,yshift=68mm,anchor=north west,inner sep = 2pt](B){
		\begin{minipage}[t]{3.5cm}
		\begin{center}
			Academic Partners \\[.5cm]
			\adjincludegraphics[trim=0mm 0cm 0mm 0cm,clip,width=35mm]{EJLateX/img//CEUR.jpg}\\[.5cm]
			\adjincludegraphics[trim=0mm 0cm 0mm 0cm,clip,width=35mm]{EJLateX/img/novauniversitas.png}
		\end{center}
		\end{minipage}
	};

\end{tikzpicture}

\clearpage


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% second cover %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\thispagestyle{plain}

\vspace*{-30pt}%
\vspace*{.07cm}
%	\begin{minipage}[t]{11.9cm}
%%		\vspace*{-34pt}
%		\hspace{-9mm}
%%			%\includegraphics[scale=1]{EJLateX/img/EJournal.png}
%%			%the following line must be blank
%			
%%			\vspace{.6cm}
%%			\hspace{-8.5mm}
%	\end{minipage}
%	\hfill
%	\hspace{1.1cm}


\hfill
\begin{minipage}[t][]{3.98cm}
	\includegraphics[scale=.16]{EJLateX/img/Euresis_Logo_big.pdf} 
\end{minipage}
\hspace{-0.7cm}

\vspace{30pt}
\begin{tikzpicture}[remember picture,overlay]
	\node at (current page.north east) [anchor=south,xshift=-5.8cm](a){};
	\node at (a) [yshift=-28cm,rectangle,draw=EJblue,fill=EJblue,scale=.8,anchor=north](b){};
	\draw[gborder, line width=1.5pt] (a) -- (b);
	\node at (current page.south west) [] (c){};
	\node at (c)[xshift=5.8cm,yshift=\paperheight )](d){};
	\draw[fill=gborderB,line width=0pt,draw=gborderB] (c) rectangle (d);	
\end{tikzpicture}


\hfill
%\begin{flushright}
%\hspace{2.8cm}
\begin{minipage}[t][0.9\textheight]{4cm}
%\begin{fullwidth}[width=4cm,skipabove=0pt,skipbelow=0pt,splittopskip=0pt,innertopmargin=0pt,innerbottommargin=-3cm]
	\begin{spacing}{.5}
	\textbf{\scriptsize  Cover image}\par\vspace{1mm}%\\[1mm]
	{\tiny \EJthiscoverdesc}
	\end{spacing}
	\vfill
	%\vspace{1cm}
	\textbf{\scriptsize  Editors}\par\vspace{2mm}
	\begin{spacing}{.5}
	{\scriptsize  Ulisses Barres de Almeida\par}
	%\textit{\tiny Max-Planck-Institut fuer Physik\\
	\textit{\tiny Centro Brasileiro de Pesquisas \\ Fisicas\\ulisses@cbpf.br}
	%ulisses@mppmu.mpg.de\\}
	\end{spacing}

	\vspace{6mm}
	\begin{spacing}{.5}
	{\scriptsize  Juan Rojo\par}
	\textit{\tiny TH Unit, PH Division, CERN\\ juan.rojo@cern.ch}\par
	\end{spacing}
	\vspace{5mm}
	{\scriptsize  journal@euresis.org}\par
	\vspace{6mm}
	\begin{spacing}{.6}
	\textbf{\scriptsize  Academic Partners}\par
	{\scriptsize Fondazione CEUR}\par
	{\scriptsize  Consortium Nova Universitas}\par
	\end{spacing}
	\vspace{1.5cm}
	\begin{spacing}{.8}
	{\footnotesize Copyright {\small \textcopyright}2012 by \\Associazione EURESIS}
	\end{spacing}
	\vspace{6mm}
	\begin{spacing}{.5}
	{\tiny The user may not modify, copy, reproduce, retransmit or otherwise distribute this publication and its contents (whether text, graphics or original research content), without express permission in writing from the Editors. Where the above content is directly or indirectly reproduced in an academic context, this must be acknowledge with the appropriate bibliographical citation. The opinions stated in the papers of the Euresis Journal are those of their respective authors and do not necessarily reflect the opinions of the Editors or the members of the Euresis Association or its sponsors.}

	\vspace{6mm}
	{\tiny Euresis Journal (ISSN 2239-2742), a publication of  Associazione Euresis, an Association for the Promotion of Scientific Endevour, Via Caduti di Marcinelle 2, 20134 Milano, Italia.\\www.euresisjournal.org}
	\vspace{5mm}
	%{\tiny www.euresisjournal.org\\}
	\vspace{4mm}

	{\tiny Contact information: \\[3mm]	Email. info@euresis.org \\ Tel.+39-022-1085-2225 \\	Fax. +39-022-1085-2222 }\par
	\end{spacing}
	\vspace{1.2cm}
	\begin{spacing}{.6}
	\textbf{\scriptsize  Graphic design and layout}\\{\tiny Lorenzo Morabito}\par
	\end{spacing}
	\vspace{.5cm}
	\begin{spacing}{.6}
	%\textbf{\scriptsize  \XeLaTeX\ template}\\
	\textbf{\scriptsize  Technical Editor}\\{\tiny Davide PJ Caironi}\par
	\end{spacing}
	\vspace{1.3cm}
	\begin{spacing}{.6}
	{\scriptsize  This document was created using \LaTeXe\ and \XeLaTeX\ }
	\end{spacing}
%\end{fullwidth}
\end{minipage}
%\end{flushright}
\hspace{-0.8cm}
%provare con una dim negativa per la vbox?
%\vbox{}

\clearpage




